Global solution for superlinear stochastic heat equation on $\mathbb{R}^d$ under Osgood-type conditions

We study the \textit{stochastic heat equation} (SHE) on $\R^d$ subject to a centered Gaussian noise that is white in time and colored in space.The drift term is assumed to satisfy an Osgood-type condition and the diffusion coefficient may have certain related growth. We show that there exists random field solution which do not explode in finite time. This complements and improves upon recent results on blow-up of solutions to stochastic partial differential equations.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.9~svn20110310	//
A:Osgood	main.tex	/^\\begin{assumption}\\label{A:Osgood}$/;"	l
A:initial	main.tex	/^\\begin{assumption}\\label{A:initial}$/;"	l
A:noise	main.tex	/^\\begin{assumption}\\label{A:noise}$/;"	l
D:2-smooth	main.tex	/^\\begin{definition}[Definition~3.1 of~\\cite{ondrejat:04:uniqueness}]\\label{D:2-smooth}$/;"	l
E:AppMom	main.tex	/^  \\begin{equation}\\label{E:AppMom}$/;"	l
E:BDG-Y	main.tex	/^  \\begin{align} \\label{E:BDG-Y}$/;"	l
E:Banach-BDG	main.tex	/^  \\begin{gather}\\label{E:Banach-BDG}$/;"	l
E:Claim_1	main.tex	/^  \\begin{align}\\label{E:Claim_1}$/;"	l
E:Claim_2	main.tex	/^  \\begin{gather}\\label{E:Claim_2}$/;"	l
E:Contradiction-Ass	main.tex	/^  \\begin{align}\\label{E:Contradiction-Ass}$/;"	l
E:Dalang	main.tex	/^\\begin{align}\\label{E:Dalang}$/;"	l
E:Dalang+	main.tex	/^\\begin{align}\\label{E:Dalang+}$/;"	l
E:EYp	main.tex	/^  \\begin{align}\\label{E:EYp}$/;"	l
E:General-B-BDG	main.tex	/^  \\begin{equation}\\label{E:General-B-BDG}$/;"	l
E:H-inner-Prod	main.tex	/^\\begin{equation}\\label{E:H-inner-Prod}$/;"	l
E:Iterate-b	main.tex	/^  \\begin{equation}\\label{E:Iterate-b}$/;"	l
E:Iterate-s	main.tex	/^  \\begin{equation}\\label{E:Iterate-s}$/;"	l
E:Lr	main.tex	/^  \\begin{equation}\\label{E:Lr}$/;"	l
E:Max-Doob	main.tex	/^  \\begin{align}\\label{E:Max-Doob}$/;"	l
E:Mild	main.tex	/^\\begin{equation}\\label{E:Mild}$/;"	l
E:Noise	main.tex	/^\\begin{equation}\\label{E:Noise}$/;"	l
E:ODE	main.tex	/^\\begin{align}\\label{E:ODE}$/;"	l
E:Osgood-Fnt	main.tex	/^\\begin{align}\\label{E:Osgood-Fnt}$/;"	l
E:Osgood-Inf	main.tex	/^\\begin{align}\\label{E:Osgood-Inf}$/;"	l
E:Radonfiying-Lp	main.tex	/^    \\begin{equation}\\label{E:Radonfiying-Lp}$/;"	l
E:SHE	main.tex	/^\\begin{equation}\\label{E:SHE}$/;"	l
E:Stable	main.tex	/^  \\begin{equation}\\label{E:Stable}$/;"	l
E:Step-1	main.tex	/^  \\begin{align}\\label{E:Step-1}$/;"	l
E:Step-2	main.tex	/^  \\begin{align}\\label{E:Step-2}$/;"	l
E:Stopping	main.tex	/^  \\begin{equation}\\label{E:Stopping}$/;"	l
E:Y-Finite	main.tex	/^  \\begin{align}\\label{E:Y-Finite}$/;"	l
E:YDM	main.tex	/^  \\begin{gather}\\label{E:YDM}$/;"	l
E:YDM_2	main.tex	/^  \\begin{gather}\\label{E:YDM_2}$/;"	l
E:Z-bound	main.tex	/^  \\begin{align}\\label{E:Z-bound}$/;"	l
E:an-def	main.tex	/^  \\begin{equation}\\label{E:an-def}$/;"	l
E:bsigma-inf	main.tex	/^  \\begin{equation}\\label{E:bsigma-inf}$/;"	l
E:exp-moment	main.tex	/^  \\begin{align}\\label{E:exp-moment}$/;"	l
E:exponential-estimate	main.tex	/^  \\begin{equation}\\label{E:exponential-estimate}$/;"	l
E:factor-Y	main.tex	/^    Y(r,z) = & \\int_0^r \\int_{\\R^d} (r-s)^{-\\beta\/2} p_{r-s}(z-y) \\Phi(s,y) W(\\ud s,\\ud y). \\label{E:factor-Y}$/;"	l
E:factor-Z	main.tex	/^  \\begin{align} \\label{E:factor-Z}$/;"	l
E:factored-moment	main.tex	/^  \\begin{align}\\label{E:factored-moment}$/;"	l
E:new-osgood	main.tex	/^          \\begin{equation}\\label{E:new-osgood}$/;"	l
E:quad-var	main.tex	/^  \\begin{align}\\label{E:quad-var}$/;"	l
E:stopping-times	main.tex	/^  \\begin{align}\\label{E:stopping-times}$/;"	l
E:u_0-Theta	main.tex	/^  \\begin{align}\\label{E:u_0-Theta}$/;"	l
L:Banach-BDG	main.tex	/^\\begin{lemma}\\label{L:Banach-BDG}$/;"	l
L:Iterate	main.tex	/^\\begin{lemma}\\label{L:Iterate}$/;"	l
L:Lr	main.tex	/^\\begin{lemma}\\label{L:Lr}$/;"	l
L:Stable	main.tex	/^\\begin{lemma}\\label{L:Stable}$/;"	l
L:exponential-estimate	main.tex	/^\\begin{lemma}[Exponential estimates]\\label{L:exponential-estimate}$/;"	l
S:BDG	main.tex	/^\\section{Appendix}\\label{S:BDG}$/;"	l
S:Example	main.tex	/^\\section{An explosion example---the proof of Theorem~\\ref{T:Ex-Blowup}}\\label{S:Example}$/;"	l
S:Main	main.tex	/^\\section{Proof of Theorem~\\ref{T:Main}}\\label{S:Main}$/;"	l
S:Prelim	main.tex	/^\\section{Some preliminaries}\\label{S:Prelim}$/;"	l
T:Banach-BDG	main.tex	/^\\begin{theorem}\\label{T:Banach-BDG}$/;"	l
T:Ex-Blowup	main.tex	/^\\begin{theorem}\\label{T:Ex-Blowup}$/;"	l
T:Main	main.tex	/^\\begin{theorem}\\label{T:Main}$/;"	l
T:Moment	main.tex	/^\\begin{theorem}[Moment formulas under Lipschitz condition]\\label{T:Moment}$/;"	l
Tb:Bdd	main.tex	/^    \\label{Tb:Bdd}$/;"	l
Tb:Eg	main.tex	/^  \\label{Tb:Eg}$/;"	l
Tb:General	main.tex	/^    \\label{Tb:General}$/;"	l
Tb:ST-White-1D	main.tex	/^    \\label{Tb:ST-White-1D}$/;"	l
athreya.joseph.ea:21:small	main_biber.bib	/^@ARTICLE{athreya.joseph.ea:21:small,$/;"	b
cerrai.rockner:04:large	main_biber.bib	/^@ARTICLE{cerrai.rockner:04:large,$/;"	b
chen.huang:19:comparison	main_biber.bib	/^@ARTICLE{chen.huang:19:comparison,$/;"	b
chen.huang:23:superlinear	main_biber.bib	/^@ARTICLE{chen.huang:23:superlinear,$/;"	b
dalang.khoshnevisan.ea:09:minicourse	main_biber.bib	/^@BOOK{dalang.khoshnevisan.ea:09:minicourse,$/;"	b
dalang.khoshnevisan.ea:19:global	main_biber.bib	/^@ARTICLE{dalang.khoshnevisan.ea:19:global,$/;"	b
dalang:99:extending	main_biber.bib	/^@ARTICLE{dalang:99:extending,$/;"	b
fernandez-bonder.groisman:09:time-space	main_biber.bib	/^@ARTICLE{fernandez-bonder.groisman:09:time-space,$/;"	b
foondun.nualart:21:osgood	main_biber.bib	/^@ARTICLE{foondun.nualart:21:osgood,$/;"	b
foondun.nualart:22:non-existence	main_biber.bib	/^@ARTICLE{foondun.nualart:22:non-existence,$/;"	b
fujita:66:on	main_biber.bib	/^@ARTICLE{fujita:66:on,$/;"	b
gei.manthey:94:comparison	main_biber.bib	/^@ARTICLE{gei.manthey:94:comparison,$/;"	b
khoshnevisan:14:analysis	main_biber.bib	/^@BOOK{khoshnevisan:14:analysis,$/;"	b
millet.sanz-sole:21:global	main_biber.bib	/^@ARTICLE{millet.sanz-sole:21:global,$/;"	b
mueller:91:on	main_biber.bib	/^@ARTICLE{mueller:91:on,$/;"	b
olver.lozier.ea:10:nist	main_biber.bib	/^@BOOK{olver.lozier.ea:10:nist,$/;"	b
ondrejat:04:uniqueness	main_biber.bib	/^@ARTICLE{ondrejat:04:uniqueness,$/;"	b
osgood:98:beweis	main_biber.bib	/^@ARTICLE{osgood:98:beweis,$/;"	b
quittner.souplet:19:superlinear	main_biber.bib	/^@BOOK{quittner.souplet:19:superlinear,$/;"	b
salins:22:existence	main_biber.bib	/^@ARTICLE{salins:22:existence,$/;"	b
salins:22:global	main_biber.bib	/^@ARTICLE{salins:22:global,$/;"	b
salins:22:global*1	main_biber.bib	/^@ARTICLE{salins:22:global*1,$/;"	b
seidler:10:exponential	main_biber.bib	/^@ARTICLE{seidler:10:exponential,$/;"	b
shang.zhang:21:global	main_biber.bib	/^@ARTICLE{shang.zhang:21:global,$/;"	b
shang.zhang:22:stochastic	main_biber.bib	/^@ARTICLE{shang.zhang:22:stochastic,$/;"	b
walsh:86:introduction	main_biber.bib	/^@INCOLLECTION{walsh:86:introduction,$/;"	b
zhang:10:stochastic	main_biber.bib	/^@ARTICLE{zhang:10:stochastic,$/;"	b

